NotNets: Accelerating Microservices by Bypassing the Network

Remote procedure calls are the workhorse of distributed systems. However, as software engineering trends, such as micro-services and serverless computing, push applications towards ever finer-grained decompositions, the overhead of RPC-based communication is becoming too great to bear. In this paper, we argue that point solutions that attempt to optimize one aspect of RPC logic are unlikely to mitigate these ballooning communication costs. Rather, we need a dramatic reappraisal of how we provide communication. Towards this end, we propose to emulate message-passing RPCs by sharing message payloads and metadata on CXL 3.0-backed far memory. We provide initial evidence of feasibility and analyze the expected benefits.

==> config.tex <==

% Color
\usepackage{xcolor}
\definecolor{pennblue}{cmyk}{1,.65,0,.3}
\definecolor{pennred}{cmyk}{0,1,.65,.34}

% https://latexcolor.com
% https://www.datylon.com/blog/data-visualization-for-colorblind-readers
\definecolor{bananamania}{rgb}{0.98, 0.91, 0.71} % #FAE7B5
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94} % #89CFF0

\newcommand{\todo}[1]{\textit{\textcolor{red}{[TODO]: #1}}}
\newcommand{\pa}[1]{\textit{\textcolor{blue}{[pa]: #1}}}
\newcommand{\rjs}[1]{\textit{\textcolor{red}{[rjs]: #1}}}

\newcommand{\cutme}[1]{\textit{\textcolor{blue}{[CUT?]: #1}}}

\newcommand{\PAR}[1]{\par\smallskip\noindent\textbf{#1}}




\usepackage{alltt}
\usepackage{wrapfig}
\usepackage{cmtt}
\usepackage{paralist}
\usepackage{lastpage}
\usepackage{times}
\usepackage{tikz}
\usepackage{balance}

\usepackage{caption}
\usepackage{subcaption}
\usepackage{xspace}
\usepackage{comment}

\usepackage{enumitem}
\newcommand{\subscript}[2]{$#1 _ #2$}

\graphicspath{{./figures/}{../figures/}}

\usepackage{url}

\usepackage{booktabs}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

\usepackage{listings}
\usepackage{multicol}

\usepackage{url,fullpage,cite,epsfig,xspace,mathpazo,kpfonts,multirow,dcolumn,colortbl,wasysym,pifont,xspace}
%\usepackage[hang,small,bf]{caption}
\usepackage[T1]{fontenc}

